RFEye in the Sky

We introduce RFEye, a generalized technique to locate signals independent of the waveform, using a single Unmanned Aerial Vehicle (UAV) equipped with only one omnidirectional antenna. This is achieved by acquiring signals from uncoordinated positions within a sphere of 1-meter radius at two nearby locations and formulating an asynchronous, distributed receiver beamforming at the UAV to compute the Direction of Arrival (DoA) from the unknown transmitter. The proposed method includes four steps: 1) Blind detection and extraction of unique signature in the signal to be localized, 2) Asynchronous signal acquisition and conditioning, 3) DoA calculation by creating a virtual distributed antenna array at UAV and 4) Obtaining position fix of emitter using DoA from two locations. These steps are analyzed for various sources of error, computational complexity and compared with widely used signal subspace-based DoA estimation algorithms. RFEye is implemented using an Intel-Aero UAV, equipped with a USRP B205 software-defined radio to acquire signals from a ground emitter. Practical outdoor experiments show that RFEye achieves a median accuracy of 1.03m in 2D and 2.5m in 3D for Wi-Fi, and 1.15m in 2D and 2.7m in 3D for LoRa (Long Range) waveforms, and is robust to external factors like wind and UAV position errors.

==> abstract.tex <==
\IEEEtitleabstractindextext{%
\begin{abstract}

We introduce {\abbrev}, a generalized technique to locate signals independent of the waveform, using a single Unmanned Aerial Vehicle (UAV) equipped with only one omnidirectional antenna. This is achieved by acquiring signals from uncoordinated positions within a sphere of 1-meter radius at two nearby locations and formulating an asynchronous, distributed receiver beamforming at the UAV to compute the Direction of Arrival (DoA) from the unknown transmitter. The proposed method includes four steps: 1) Blind detection and extraction of unique signature in the signal to be localized, 2) Asynchronous signal acquisition and conditioning, 3) DoA calculation by creating a virtual distributed antenna array at UAV and 4) Obtaining position fix of emitter using DoA from two locations. These steps are analyzed for various sources of error, computational complexity and compared with widely used signal subspace-based DoA estimation algorithms. {\abbrev} is implemented using an Intel-Aero UAV, equipped with a USRP B205 software-defined radio to acquire signals from a ground emitter. Practical outdoor experiments show that {\abbrev} achieves a median accuracy of 1.03m in 2D and 2.5m in 3D for Wi-Fi, and 1.15m in 2D and 2.7m in 3D for LoRa (\note{Long Range}) waveforms, and is robust to external factors like wind and UAV position errors.


% We introduce {\abbrev}, a generalized technique to locate signals independent of the waveform, using a single Unmanned Aerial Vehicle (UAV) equipped with only one omnidirectional antenna. This is achieved by acquiring signals from uncoordinated positions within a sphere of 1 meter radius at two nearby locations and employing an asynchronous, distributed receiver beamforming at the UAV to compute the Direction of Arrival (DoA) from the unknown transmitter. The proposed method includes four steps: 1) Blind detection and extraction of an unique signature in the radio signal to be localized, 2) Asynchronous signal acquisition and conditioning, 3) DoA calculation by creating a virtual distributed antenna array at the UAV and 4) Obtain position fix of the emitter using the DoA from two locations. These steps are analyzed for various sources of error, computational complexity and compared with widely used signal subspace based DoA estimation algorithms. {\abbrev} is implemented using an Intel Aero UAV, equipped with a USRP B205 mini software-defined radio to acquire signals from a ground emitter. Practical outdoor experiments show that {\abbrev} achieves a median accuracy of $1.03m$ in 2D and $2.5m$ in 3D for Wi-Fi, and $1.15m$ in 2D and $2.7m$ in 3D for LoRa waveforms, and is robust to external factors like wind and position errors of the UAV.

%The need for precise and fast localization of radio frequency signals in the wild is crucial in search and rescue operations, detecting violation of spectrum policies and isolating RF emitters in electronic warfare. 
% We introduce {\abbrev}, a generalized technique to locate signals independent of the waveform, using a single Unmanned Aerial Vehicle (UAV) equipped with only one omnidirectional antenna. This is achieved by acquiring signals from uncoordinated positions within a sphere of approximately 1 meter in radius at no more than two nearby locations and employing an asynchronous, distributed receiver beamforming at the UAV to compute the Direction of Arrival (DoA) from the unknown transmitter.
% The proposed method includes four sequential steps: 1) Blind detection and extraction of an unique signature in the radio signal to be localized, 2) Asynchronous signal acquisition and conditioning from two nearby locations, 3) DoA calculation by creating a virtual distributed antenna array at the UAV and 4) Obtain position fix of the emitter using the DoA from two locations. Each of these steps are analyzed for various sources of error, computational complexity and compared with widely used signal subspace based DoA estimation algorithms. {\abbrev} is implemented using an Intel Aero UAV, equipped with a USRP B205 mini %Software Defined Radio (SDR) 
% software-defined radio to acquire signals from a ground emitter. Practical outdoor experiments show that {\abbrev} achieves a median accuracy of $1.03m$ in 2D and $2.5m$ in 3D for Wi-Fi waveforms, and $1.15m$ in 2D and $2.7m$ in 3D for LoRa waveforms, and is robust to external factors like wind and position errors of the UAV.



\end{abstract}
% Note that keywords are not normally used for peerreview papers.
\begin{IEEEkeywords}
Computer Society, IEEE, IEEEtran, journal, \LaTeX, paper, template.
\end{IEEEkeywords}}
